A Particle-in-cell Method for Plasmas with a Generalized Momentum Formulation, Part I: Model Formulation

This paper formulates a new particle-in-cell method for the Vlasov-Maxwell system. Under the Lorenz gauge condition, Maxwell's equations for the electromagnetic fields can be written as a collection of scalar and vector wave equations. The use of potentials for the fields motivates the adoption of a Hamiltonian formulation for particles that employs the generalized momentum. The resulting updates for particles require only knowledge of the fields and their spatial derivatives. An analytical method for constructing these spatial derivatives is presented that exploits the underlying integral solution used in the field solver for the wave equations. Moreover, these derivatives are shown to converge at the same rate as the fields in the both time and space. The field solver we consider in this work is first-order accurate in time and fifth-order accurate in space and belongs to a larger class of methods which are unconditionally stable, can address geometry, and leverage fast summation methods for efficiency. We demonstrate the method on several well-established benchmark problems, and the efficacy of the proposed formulation is demonstrated through a comparison with standard methods presented in the literature. The new method shows mesh-independent numerical heating properties even in cases where the plasma Debye length is close to the grid spacing. The use of high-order spatial approximations in the new method means that fewer grid points are required in order to achieve a fixed accuracy. Our results also suggest that the new method can be used with fewer simulation particles per cell compared to standard explicit methods, which permits further computational savings.

==> 3-Field-Solvers/boundary-conditions.tex <==
%
% Applying boundary conditions for the different schemes
%
\subsection{Applying Boundary Conditions}
\label{subsec:applying BCs}

In this section, we discuss the application of boundary conditions for the proposed method, which is based on a first-order BDF time discretization of a second time derivative. Boundary conditions are presented from the perspective of one-dimensional problems and are applied in a dimension-by-dimension fashion in multi-dimensional problems.

To set the stage for the ensuing discussion, note that the semi-discrete update for the first-order BDF method, in one-spatial dimension, can be obtained by combining \eqref{eq:1d MHE general solution 2} with the semi-discrete equation \eqref{eq:BDF-1 semi-discrete equation}. Defining the operand
\begin{equation*}
    R(x) = 2 u^{n}(x) - u^{n-1}(x) + \frac{1}{\alpha^2} S^{n+1}(x),
\end{equation*}
we obtain the update
\begin{align}
    u^{n+1}(x) &= \frac{\alpha}{2} \int_{a}^{b} e^{-\alpha \lvert x - y \rvert} R(y) \,dy + A e^{-\alpha (x - a)} + B e^{-\alpha (b - x)}, \label{eq:BDF-1 update in 1-D} \\
            &\equiv \mathcal{I}_{x}[R](x) + A e^{-\alpha (x - a)} + B e^{-\alpha (b - x)}, \label{eq:BDF-1 update in 1-D compact}
\end{align}
where we have used $\mathcal{I}_{x}[\cdot]$ to denote the term involving the convolution integral which is not to be confused with the identity operator. Applying different boundary conditions amounts to determining the values of $A$ and $B$ used in \eqref{eq:BDF-1 update in 1-D compact}. In the description of boundary conditions for the method, we shall assume that the boundary conditions at the ends of the one-dimensional domain are the same. Using slight variations of the methods illustrated below, one can mix the boundary conditions at the ends of the line segments.

In order to enforce conditions on the derivatives of the solution, we will also need to compute a derivative of the update \eqref{eq:BDF-1 update in 1-D} (equivalently \eqref{eq:BDF-1 update in 1-D compact}). For this, we observe that the dependency for $x$ appears only on analytical functions, i.e., the Green's function (kernel) and the exponential functions in the boundary terms. To differentiate \eqref{eq:BDF-1 update in 1-D} we start with the definition \eqref{eq:Average of IR and IL}, which splits the integral at the point $y = x$ and makes the kernel easier to manipulate. Then, using the fundamental theorem of calculus, we can calculate derivatives of
\eqref{eq:right integral of operand} and \eqref{eq:left integral of operand} to find that
\begin{align}
    \frac{d}{dx} \left( \mathcal{I}_{x}^{R}[f](x) \right) =  \frac{d}{dx} \left( \alpha \int_{a}^{x} e^{-\alpha (x - y)} f(y) \,dy \right) = -\alpha \mathcal{I}_{x}^{R}[f](x) + \alpha f(x), \label{eq:ddx right integral of operand} \\
    \frac{d}{dx} \left(
    \mathcal{I}_{x}^{L}[f](x) \right) = \frac{d}{dx} \left( \alpha \int_{x}^{b} e^{-\alpha (y - x)} f(y) \,dy \right) =
    \alpha \mathcal{I}_{x}^{L}[f](x) - \alpha f(x), \label{eq:ddx left integral of operand}
\end{align}
These results can be combined according to \eqref{eq:Average of IR and IL}, which provides an expression for the derivative of the convolution term:
\begin{equation}
    \label{eq:ddx of convolution}
    \frac{d}{dx} \Big( \mathcal{I}_{x}[f](x) \Big) = \frac{\alpha}{2} \Big( - \mathcal{I}_{x}^{R}[f](x) +  \mathcal{I}_{x}^{L}[f](x) \Big).
\end{equation}
Additionally, by evaluating this equation at the ends of the interval, we obtain the identities
\begin{align}
    \frac{d}{dx} \Big( \mathcal{I}_{x}[f](a) \Big)  &= \alpha  \mathcal{I}_{x}[f](a), \label{eq:ddx of convolution at a} \\
    \frac{d}{dx} \Big( \mathcal{I}_{x}[f](b) \Big)  &= -\alpha  \mathcal{I}_{x}[f](b), \label{eq:ddx of convolution at b}
\end{align}
which are helpful in enforcing the boundary conditions. The relation \eqref{eq:ddx of convolution} can be used to obtain a derivative for the solution at the new time level. From the update \eqref{eq:BDF-1 update in 1-D compact}, a direct computation reveals that
\begin{equation}
    \label{eq:BDF-1 ddx update in 1-D}
    \frac{d  u^{n+1}}{dx} = \frac{\alpha}{2} \left( - \mathcal{I}_{x}^{R}[R](x) +  \mathcal{I}_{x}^{L}[R](x) \right) -\alpha A e^{-\alpha (x-a)} + \alpha B e^{-\alpha (b-x)}.
\end{equation}
Notice that no additional approximations have been made beyond what is needed to compute $\mathcal{I}_{x}^{R}$ and $\mathcal{I}_{x}^{L}$. These terms are already evaluated as part of the base method. For this reason, we think of equation \eqref{eq:BDF-1 ddx update in 1-D} as an analytical derivative. The boundary coefficients $A$ and $B$ appearing in \eqref{eq:BDF-1 ddx update in 1-D} will be calculated in the same way as the update \eqref{eq:BDF-1 update in 1-D compact}, and are discussed in the remaining subsections. This treatment ensures that the discrete derivative will be consistent with the conditions imposed on the solution variable.


\subsubsection{Dirichlet Boundary Conditions}
\label{subsubsec:BDF-1 Dirichlet}

Suppose we are given the function values along the boundary, which is represented by the data
\begin{equation*}
    u^{n+1}(a) = g_{a} \left(t^{n+1}\right), \quad u^{n+1}(b) = g_{b} \left(t^{n+1}\right).
\end{equation*}
If we evaluate the BDF-1 update \eqref{eq:BDF-1 update in 1-D compact} at the ends of the interval, we obtain the conditions
\begin{align*}
    g_{a} \left(t^{n+1}\right) &= \mathcal{I}_{x}[R](a) + A + \mu B, \\
    g_{b} \left(t^{n+1}\right) &= \mathcal{I}_{x}[R](b) + \mu A + B,
\end{align*}
where we have defined $\mu = e^{-\alpha(b-a)}$. This is a simple linear system for the boundary coefficients $A$ and $B$, which can be inverted by hand. Proceeding, we find that
\begin{align*}
    A &= \frac{g_{a} \left(t^{n+1}\right) - \mathcal{I}_{x}[R](a) - \mu \left( g_{b} \left(t^{n+1}\right) - \mathcal{I}_{x}[R](b) \right)}{1 - \mu^2}, \\
    B &= \frac{g_{b} \left(t^{n+1}\right) - \mathcal{I}_{x}[R](b) - \mu \left( g_{a} \left(t^{n+1}\right) - \mathcal{I}_{x}[R](a) \right)}{1 - \mu^2}.
\end{align*}


\subsubsection{Neumann Boundary Conditions}
\label{subsubsec:BDF-1 Neumann}

We can also enforce conditions on the derivatives at the end of the domain. Given the Neumann data
\begin{equation*}
    \frac{d u^{n+1}(a)}{dx} = h_{a} \left(t^{n+1}\right), \quad \frac{d  u^{n+1}(b)}{dx} = h_{b} \left(t^{n+1}\right),
\end{equation*}
we can evaluate the derivative formula for the update \eqref{eq:BDF-1 ddx update in 1-D} and use the identities \eqref{eq:ddx of convolution at a} and \eqref{eq:ddx of convolution at b}. Performing these evaluations, we obtain the system of equations
\begin{align*}
    -A + \mu B &= \frac{1}{\alpha} h_{a} \left(t^{n+1}\right) - \mathcal{I}_{x}[R](a), \\
    -\mu A + B &= \frac{1}{\alpha} h_{b} \left(t^{n+1}\right) + \mathcal{I}_{x}[R](b),
\end{align*}
where, again, $\mu = e^{-\alpha(b-a)}$. Solving this system, we find that
\begin{align*}
    A &= -\frac{\frac{1}{\alpha} h_{a} \left(t^{n+1}\right) - \mathcal{I}_{x}[R](a) - \mu \left( \frac{1}{\alpha} h_{b} \left(t^{n+1}\right) + \mathcal{I}_{x}[R](b) \right)}{1-\mu^2}, \\
    B &= -\frac{ \mu \left( \frac{1}{\alpha} h_{a} \left(t^{n+1}\right) - \mathcal{I}_{x}[R](a) \right) - \left( \frac{1}{\alpha} h_{b} \left(t^{n+1}\right) + \mathcal{I}_{x}[R](b) \right)}{1-\mu^2}. 
\end{align*}
We note that Robin boundary conditions, which combine Dirichlet and Neumann conditions can be enforced in a nearly identical manner.  


\subsubsection{Periodic Boundary Conditions}
\label{subsubsec:BDF-1 periodic}

Periodic boundary conditions are enforced by taking
\begin{equation*}
    u^{n+1}(a) = u^{n+1}(b), \quad \partial_{x} u^{n+1}(a) = \partial_{x} u^{n+1}(b).
\end{equation*}
Enforcing these conditions through the update \eqref{eq:BDF-1 update in 1-D compact} and its derivative \eqref{eq:BDF-1 ddx update in 1-D}, using the identities \eqref{eq:ddx of convolution at a}-\eqref{eq:ddx of convolution at b}, leads to the system of equations
\begin{align*}
    (1 - \mu)A + (\mu - 1)B &= \mathcal{I}_{x}[R](b) - \mathcal{I}_{x}[R](a), \\
    (\mu - 1)A + (\mu - 1)B &= -\mathcal{I}_{x}[R](b) - \mathcal{I}_{x}[R](a),
\end{align*}
with $\mu = e^{-\alpha(b-a)}$. The solution of this system, after some simplifications is given by
\begin{align*}
    A &= \frac{\mathcal{I}_{x}[R](b)}{1-\mu}, \\
    B &= \frac{\mathcal{I}_{x}[R](a)}{1-\mu}. 
\end{align*}

% \subsubsection{Outflow Boundary Conditions (Do we REALLY need this???)}
% \label{subsubsec:BDF-1 outflow}

% In problems defined over free-space, we must allow for waves to exit the computational domain. Additionally, as the waves exit the domain, we would like to minimize the number of reflections, which are non-physical, along this boundary. Exit conditions can be formulated in one-dimension in the sense of characteristics, by requiring that
% \begin{align}
%     \frac{\partial u}{\partial t} - c \frac{\partial u}{\partial x} &= 0, \quad x = a, \label{eq:Outflow left condition} \\
%     \frac{\partial u}{\partial t} + c \frac{\partial u}{\partial x} &= 0, \quad x = b, \label{eq:Outflow right condition}
% \end{align}
% where $c > 0$ is the wave speed. 

% To formulate the boundary conditions for the first-order BDF update \eqref{eq:BDF-1 update in 1-D}, we follow the approach used in \cite{causley2017wave-propagation}. This paper developed outflow boundary conditions for a variant of the proposed solver, in which the time derivatives are discretized with time-centered stencils. The development of outflow boundary conditions starts from the free-space solution that is defined over the real line:
% \begin{equation*}
%     u^{n+1}(x) = \frac{\alpha}{2} \int_{-\infty}^{\infty} e^{-\alpha \lvert x - y \rvert} R(y) \, dy.
% \end{equation*}
% Here, $R(x)$ is the operand for the BDF-1 method given by (ignoring sources)
% \begin{equation*}
%     R(x) = 2 u^{n} - u^{n-1}.
% \end{equation*}
% Using the finite speed of propagation and assuming that the support of $u(x,0)$ and $R(x)$ is entirely contained within the domain $[a,b]$, it follows that the free-space solution can be written in the familiar form \eqref{eq:BDF-1 update in 1-D compact}:
% \begin{equation*}
%      u^{n+1}(x) = \mathcal{I}_{x}[R](x) + A^{n} e^{-\alpha (x-a)} + B^{n} e^{-\alpha (b-x)}.
% \end{equation*}
% In the above, we have employed the definitions
% \begin{align}
% A^{n} &= \frac{\alpha}{2} \int_{a - c t^{n}}^{a} e^{-\alpha(a-y)}R(y)\,dy, \label{eq:Free-space A finite} \\
% B^{n} &= \frac{\alpha}{2} \int_{b}^{b + c t^{n}} e^{-\alpha(y-b)}R(y)\,dy. \label{eq:Free-space B finite}
% \end{align}
% Since these integrals are defined over regions of space outside of the computational domain, the idea is now to exchange space with time, using the characteristics of equations \eqref{eq:Outflow left condition} and \eqref{eq:Outflow right condition}. 

% A key difference between the BDF and time-centered approaches is the definition of the operand in the convolution operators. In the time centered approach, the operand consists of a single time level $u^{n}(x)$, while the BDF methods use additional time levels, e.g., $u^{n-1}(x)$, $u^{n-2}(x)$, etc; however, the outflow approach developed for the time-centered method \cite{causley2017wave-propagation} can still be used in the BDF method. Through Taylor expansion, it is straightforward to verify that
% \begin{equation}
%     \label{eq:Taylor expansion of BDF operand}
%     2u^{n}(x) - u^{n-1}(x) = u^{n} + \partial_{t} u^{n}(x)\Delta t + \mathcal{O}(\Delta t^2).
% \end{equation}
% The linearization \eqref{eq:Taylor expansion of BDF operand}, which is used only along the boundary points, turns out to be quite effective for problems with slow variations in time as well as steady-state problems. The Taylor expansion shows that in such situations, the time derivatives become small so that higher-order terms can be neglected. Therefore, if we approximate the operand $R$ along the boundary $x = b$ with $u \left(b, t^{n} - y \right)$, it follows that
% \begin{align*}
%     B^{n} &= \frac{\alpha c}{2} \int_{0}^{t^{n}} e^{-\alpha c y} u \left(b, t^{n} - y \right) \,dy, \\
%     &= \frac{\alpha c}{2} \int_{0}^{\Delta t} e^{-\alpha c y} u \left(b, t^{n} - y \right) \,dy + \frac{\alpha c}{2} \int_{\Delta t}^{t^{n}} e^{-\alpha c y} u \left(b, t^{n} - y \right) \,dy, \\
%     &\equiv I_{1} + I_{2},
% \end{align*}
% where the second integral $I_{2}$ can be written in the form
% \begin{align}
%     I_{2} &= \frac{\alpha c}{2} \int_{0}^{t^{n-1}} e^{-\alpha c (y + \Delta t)} u \left(b, t^{n-1} - y \right) \,dy, \nonumber \\ 
%     &= e^{-1} \left( \frac{\alpha c}{2} \int_{0}^{t^{n-1}} e^{-\alpha c y} u \left(b, t^{n-1} - y \right) \,dy \right), \nonumber \\
%     &\equiv e^{-1} B^{n-1}.  \label{eq:I_2 outflow simplified for central-2}
% \end{align}
% Note that the simplifications shown above use the definition $\alpha = 1/(c \Delta t)$ for the BDF-1 method.

% Likewise, the first integral $I_{1}$, can be expressed as
% \begin{equation}
%     I_{1} = \frac{1}{2} \int_{0}^{1} e^{- z}  u \left(b, t^{n} - z\Delta t \right) \,dz, \label{eq:I_1 outflow simplified central-2}
% \end{equation}
% using the definition $\alpha = 1/(c \Delta t)$. As with the BDF-1 method, this integral can be evaluated analytically after constructing an interpolating function for $u \left(b, t^{n} - z\Delta t \right)$. If we approximate the function $u \left(b, t^{n} - z\Delta t \right)$ using algebraic polynomials with the data $\{u^{n-2}(b), u^{n-1}(b), u^{n}(b)\}$ as the stencil, we obtain the coefficient
% \begin{equation*}
%     B^{n} = e^{-\beta} B^{n-1} + \gamma_{0} u^{n}(b) + \gamma_{1} u^{n-1}(b) + \gamma_{2} u^{n-2}(b),
% \end{equation*}
% where the integration weights are given by
% \begin{align*}
%     \gamma_{0} &=  \frac{2 e^{-\beta} -\beta + 2\beta^2 + 3\beta e^{-\beta} - 2}{4\beta^2}, \\
%     \gamma_{1} &= -\frac{2 e^{-\beta} -2\beta +3 \beta^2 e^{-\beta} + 4 \beta e^{-\beta} - 2}{6\beta^2}, \\
%     \gamma_{2} &= -\frac{\beta + 2e^{-\beta} + \beta e^{-\beta} - 2}{12\beta^2},
% \end{align*}
% with $\beta = 1$.






